CoMAC: Conversational Agent for Multi-Source Auxiliary Context with Sparse and Symmetric Latent Interactions

Recent advancements in AI-driven conversational agents have exhibited immense potential of AI applications. Effective response generation is crucial to the success of these agents. While extensive research has focused on leveraging multiple auxiliary data sources (e.g., knowledge bases and personas) to enhance response generation, existing methods often struggle to efficiently extract relevant information from these sources. There are still clear limitations in the ability to combine versatile conversational capabilities with adherence to known facts and adaptation to large variations in user preferences and belief systems, which continues to hinder the wide adoption of conversational AI tools. This paper introduces a novel method, Conversational Agent for Multi-Source Auxiliary Context with Sparse and Symmetric Latent Interactions (CoMAC), for conversation generation, which employs specialized encoding streams and post-fusion grounding networks for multiple data sources to identify relevant persona and knowledge information for the conversation. CoMAC also leverages a novel text similarity metric that allows bi-directional information sharing among multiple sources and focuses on a selective subset of meaningful words. Our experiments show that CoMAC improves the relevant persona and knowledge prediction accuracies and response generation quality significantly over two state-of-the-art methods.

==> figures/k_gen.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(5760.00,4320.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(444,704){\makebox(0,0)[r]{\strut{}$0.15$}}%
      \put(444,1160){\makebox(0,0)[r]{\strut{}$0.2$}}%
      \put(444,1616){\makebox(0,0)[r]{\strut{}$0.25$}}%
      \put(444,2072){\makebox(0,0)[r]{\strut{}$0.3$}}%
      \put(444,2527){\makebox(0,0)[r]{\strut{}$0.35$}}%
      \put(444,2983){\makebox(0,0)[r]{\strut{}$0.4$}}%
      \put(444,3439){\makebox(0,0)[r]{\strut{}$0.45$}}%
      \put(576,484){\makebox(0,0){\strut{}$0$}}%
      \put(1010,484){\makebox(0,0){\strut{}$1$}}%
      \put(1444,484){\makebox(0,0){\strut{}$2$}}%
      \put(1878,484){\makebox(0,0){\strut{}$3$}}%
      \put(2312,484){\makebox(0,0){\strut{}$4$}}%
      \put(2747,484){\makebox(0,0){\strut{}$5$}}%
      \put(3181,484){\makebox(0,0){\strut{}$6$}}%
      \put(3615,484){\makebox(0,0){\strut{}$7$}}%
      \put(4049,484){\makebox(0,0){\strut{}$8$}}%
      \put(4483,484){\makebox(0,0){\strut{}$9$}}%
      \put(4615,704){\makebox(0,0)[l]{\strut{}$7$}}%
      \put(4615,978){\makebox(0,0)[l]{\strut{}$8$}}%
      \put(4615,1251){\makebox(0,0)[l]{\strut{}$9$}}%
      \put(4615,1525){\makebox(0,0)[l]{\strut{}$10$}}%
      \put(4615,1798){\makebox(0,0)[l]{\strut{}$11$}}%
      \put(4615,2072){\makebox(0,0)[l]{\strut{}$12$}}%
      \put(4615,2345){\makebox(0,0)[l]{\strut{}$13$}}%
      \put(4615,2619){\makebox(0,0)[l]{\strut{}$14$}}%
      \put(4615,2892){\makebox(0,0)[l]{\strut{}$15$}}%
      \put(4615,3166){\makebox(0,0)[l]{\strut{}$16$}}%
      \put(4615,3439){\makebox(0,0)[l]{\strut{}$17$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1049,4037){\makebox(0,0)[r]{\strut{}\large F1}}%
      \csname LTb\endcsname%%
      \put(1049,3817){\makebox(0,0)[r]{\strut{}\large ROGUE1}}%
      \csname LTb\endcsname%%
      \put(2828,4037){\makebox(0,0)[r]{\strut{}\large ROGUE2}}%
      \csname LTb\endcsname%%
      \put(2828,3817){\makebox(0,0)[r]{\strut{}\large ROGUEL}}%
      \csname LTb\endcsname%%
      \put(4607,4037){\makebox(0,0)[r]{\strut{}\large BLEU}}%
      \csname LTb\endcsname%%
      \put(4607,3817){\makebox(0,0)[r]{\strut{}\large PPL$^{\downarrow}$}}%
      \csname LTb\endcsname%%
      \put(-161,2071){\rotatebox{-270.00}{\makebox(0,0){\strut{}\Large F1 / ROGUE}}}%
      \put(5121,2071){\rotatebox{-270.00}{\makebox(0,0){\strut{}\Large BLEU / PPL$^{\downarrow}$}}}%
      \put(2529,154){\makebox(0,0){\strut{}\huge $\alpha$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={288.00bp},height={216.00bp}]{gpl/k_gen}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/k_kg.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(5760.00,4320.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(444,704){\makebox(0,0)[r]{\strut{}$0.4$}}%
      \put(444,1197){\makebox(0,0)[r]{\strut{}$0.5$}}%
      \put(444,1689){\makebox(0,0)[r]{\strut{}$0.6$}}%
      \put(444,2182){\makebox(0,0)[r]{\strut{}$0.7$}}%
      \put(444,2674){\makebox(0,0)[r]{\strut{}$0.8$}}%
      \put(444,3166){\makebox(0,0)[r]{\strut{}$0.9$}}%
      \put(444,3659){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(576,484){\makebox(0,0){\strut{}$0$}}%
      \put(1045,484){\makebox(0,0){\strut{}$1$}}%
      \put(1514,484){\makebox(0,0){\strut{}$2$}}%
      \put(1983,484){\makebox(0,0){\strut{}$3$}}%
      \put(2452,484){\makebox(0,0){\strut{}$4$}}%
      \put(2921,484){\makebox(0,0){\strut{}$5$}}%
      \put(3390,484){\makebox(0,0){\strut{}$6$}}%
      \put(3859,484){\makebox(0,0){\strut{}$7$}}%
      \put(4328,484){\makebox(0,0){\strut{}$8$}}%
      \put(4797,484){\makebox(0,0){\strut{}$9$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(2721,4037){\makebox(0,0)[r]{\strut{}\large KG}}%
      \csname LTb\endcsname%%
      \put(-29,2181){\rotatebox{-270.00}{\makebox(0,0){\strut{}\Large \Large KG}}}%
      \put(2686,154){\makebox(0,0){\strut{}\huge $\alpha$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={288.00bp},height={216.00bp}]{gpl/k_kg}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/l_gen.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(5760.00,3310.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(946,825){\makebox(0,0)[r]{\strut{}$0.2$}}%
      \put(946,1166){\makebox(0,0)[r]{\strut{}$0.25$}}%
      \put(946,1506){\makebox(0,0)[r]{\strut{}$0.3$}}%
      \put(946,1847){\makebox(0,0)[r]{\strut{}$0.35$}}%
      \put(946,2187){\makebox(0,0)[r]{\strut{}$0.4$}}%
      \put(946,2528){\makebox(0,0)[r]{\strut{}$0.45$}}%
      \put(1078,537){\makebox(0,0){\strut{}$0$}}%
      \put(1962,537){\makebox(0,0){\strut{}$5$}}%
      \put(2847,537){\makebox(0,0){\strut{}$10$}}%
      \put(3731,537){\makebox(0,0){\strut{}$15$}}%
      \put(4615,537){\makebox(0,0){\strut{}$20$}}%
      \put(4747,757){\makebox(0,0)[l]{\strut{}$7$}}%
      \put(4747,961){\makebox(0,0)[l]{\strut{}$8$}}%
      \put(4747,1166){\makebox(0,0)[l]{\strut{}$9$}}%
      \put(4747,1370){\makebox(0,0)[l]{\strut{}$10$}}%
      \put(4747,1574){\makebox(0,0)[l]{\strut{}$11$}}%
      \put(4747,1779){\makebox(0,0)[l]{\strut{}$12$}}%
      \put(4747,1983){\makebox(0,0)[l]{\strut{}$13$}}%
      \put(4747,2187){\makebox(0,0)[l]{\strut{}$14$}}%
      \put(4747,2392){\makebox(0,0)[l]{\strut{}$15$}}%
      \put(4747,2596){\makebox(0,0)[l]{\strut{}$16$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1168,3137){\makebox(0,0)[r]{\strut{}F1}}%
      \csname LTb\endcsname%%
      \put(1168,2917){\makebox(0,0)[r]{\strut{}ROGUE1}}%
      \csname LTb\endcsname%%
      \put(2815,3137){\makebox(0,0)[r]{\strut{}ROGUE2}}%
      \csname LTb\endcsname%%
      \put(2815,2917){\makebox(0,0)[r]{\strut{}ROGUEL}}%
      \csname LTb\endcsname%%
      \put(4462,3137){\makebox(0,0)[r]{\strut{}BLEU}}%
      \csname LTb\endcsname%%
      \put(4462,2917){\makebox(0,0)[r]{\strut{}PPL$^{\downarrow}$}}%
      \csname LTb\endcsname%%
      \put(209,1676){\rotatebox{-270.00}{\makebox(0,0){\strut{}F1 / ROGUE}}}%
      \put(5253,1676){\rotatebox{-270.00}{\makebox(0,0){\strut{}BLEU / PPL$^{\downarrow}$}}}%
      \put(2846,207){\makebox(0,0){\strut{}\Large $\gamma$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={288.00bp},height={165.50bp}]{gpl/l_gen}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/p_gen.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(5760.00,4320.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(444,704){\makebox(0,0)[r]{\strut{}$0.15$}}%
      \put(444,1160){\makebox(0,0)[r]{\strut{}$0.2$}}%
      \put(444,1616){\makebox(0,0)[r]{\strut{}$0.25$}}%
      \put(444,2072){\makebox(0,0)[r]{\strut{}$0.3$}}%
      \put(444,2527){\makebox(0,0)[r]{\strut{}$0.35$}}%
      \put(444,2983){\makebox(0,0)[r]{\strut{}$0.4$}}%
      \put(444,3439){\makebox(0,0)[r]{\strut{}$0.45$}}%
      \put(576,484){\makebox(0,0){\strut{}$0$}}%
      \put(1010,484){\makebox(0,0){\strut{}$1$}}%
      \put(1444,484){\makebox(0,0){\strut{}$2$}}%
      \put(1878,484){\makebox(0,0){\strut{}$3$}}%
      \put(2312,484){\makebox(0,0){\strut{}$4$}}%
      \put(2747,484){\makebox(0,0){\strut{}$5$}}%
      \put(3181,484){\makebox(0,0){\strut{}$6$}}%
      \put(3615,484){\makebox(0,0){\strut{}$7$}}%
      \put(4049,484){\makebox(0,0){\strut{}$8$}}%
      \put(4483,484){\makebox(0,0){\strut{}$9$}}%
      \put(4615,704){\makebox(0,0)[l]{\strut{}$6$}}%
      \put(4615,1251){\makebox(0,0)[l]{\strut{}$8$}}%
      \put(4615,1798){\makebox(0,0)[l]{\strut{}$10$}}%
      \put(4615,2345){\makebox(0,0)[l]{\strut{}$12$}}%
      \put(4615,2892){\makebox(0,0)[l]{\strut{}$14$}}%
      \put(4615,3439){\makebox(0,0)[l]{\strut{}$16$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1049,4037){\makebox(0,0)[r]{\strut{}\large F1}}%
      \csname LTb\endcsname%%
      \put(1049,3817){\makebox(0,0)[r]{\strut{}\large ROGUE1}}%
      \csname LTb\endcsname%%
      \put(2828,4037){\makebox(0,0)[r]{\strut{}\large ROGUE2}}%
      \csname LTb\endcsname%%
      \put(2828,3817){\makebox(0,0)[r]{\strut{}\large ROGUEL}}%
      \csname LTb\endcsname%%
      \put(4607,4037){\makebox(0,0)[r]{\strut{}\large BLEU}}%
      \csname LTb\endcsname%%
      \put(4607,3817){\makebox(0,0)[r]{\strut{}\large PPL$^{\downarrow}$}}%
      \csname LTb\endcsname%%
      \put(-161,2071){\rotatebox{-270.00}{\makebox(0,0){\strut{}\Large F1 / ROGUE}}}%
      \put(5121,2071){\rotatebox{-270.00}{\makebox(0,0){\strut{}\Large BLEU / PPL$^{\downarrow}$}}}%
      \put(2529,154){\makebox(0,0){\strut{}\huge $\beta$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={288.00bp},height={216.00bp}]{gpl/p_gen}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/p_pg.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
    \definecolor{tbcol}{rgb}{1,1,1}%
\begin{picture}(5760.00,4320.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(444,704){\makebox(0,0)[r]{\strut{}$0$}}%
      \put(444,1225){\makebox(0,0)[r]{\strut{}$0.2$}}%
      \put(444,1746){\makebox(0,0)[r]{\strut{}$0.4$}}%
      \put(444,2267){\makebox(0,0)[r]{\strut{}$0.6$}}%
      \put(444,2788){\makebox(0,0)[r]{\strut{}$0.8$}}%
      \put(444,3309){\makebox(0,0)[r]{\strut{}$1$}}%
      \put(576,484){\makebox(0,0){\strut{}$0$}}%
      \put(1010,484){\makebox(0,0){\strut{}$1$}}%
      \put(1444,484){\makebox(0,0){\strut{}$2$}}%
      \put(1878,484){\makebox(0,0){\strut{}$3$}}%
      \put(2312,484){\makebox(0,0){\strut{}$4$}}%
      \put(2747,484){\makebox(0,0){\strut{}$5$}}%
      \put(3181,484){\makebox(0,0){\strut{}$6$}}%
      \put(3615,484){\makebox(0,0){\strut{}$7$}}%
      \put(4049,484){\makebox(0,0){\strut{}$8$}}%
      \put(4483,484){\makebox(0,0){\strut{}$9$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1938,4037){\makebox(0,0)[r]{\strut{}\large PG}}%
      \csname LTb\endcsname%%
      \put(1938,3817){\makebox(0,0)[r]{\strut{}\large PG-PR}}%
      \csname LTb\endcsname%%
      \put(3585,4037){\makebox(0,0)[r]{\strut{}\large PG-RC}}%
      \csname LTb\endcsname%%
      \put(3585,3817){\makebox(0,0)[r]{\strut{}\large PG-F1}}%
      \csname LTb\endcsname%%
      \put(-29,2071){\rotatebox{-270.00}{\makebox(0,0){\strut{}\Large PG Scores}}}%
      \put(2529,154){\makebox(0,0){\strut{}\huge $\beta$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics[width={288.00bp},height={216.00bp}]{gpl/p_pg}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figures/perf_change_bart_sncr.tex <==
    \begin{figure}[t!]
        \centering
        \begin{subfigure}{0.49\linewidth}
            \centering
            \begin{gnuplot}[terminal=cairolatex, scale=0.35]
                set datafile separator comma
                set key outside below
                set ytics nomirror
                set ylabel 'KG / PG'
            	plot 'figures/data/bart_sncr.csv' u 8:14 w linespoints title 'PG', \
                     'figures/data/bart_sncr.csv' u 8:16 w linespoints title 'PG-PR', \
                     'figures/data/bart_sncr.csv' u 8:17 w linespoints title 'PG-RC', \
                     'figures/data/bart_sncr.csv' u 8:(2*($16*$17)/($16+$17)) w linespoints title 'PG-F1', \
                     'figures/data/bart_sncr.csv' u 8:18 w linespoints title 'KG'
            \end{gnuplot}
            \caption{PG and KG}
            \label{fig:sncr-pg-kg}
        \end{subfigure}
        %
        \begin{subfigure}{0.49\linewidth}
            \centering
            \begin{gnuplot}[terminal=cairolatex, scale=0.35]
                set datafile separator comma
                set ylabel 'F1 / ROGUE'
                set y2tics
                set y2label 'BLEU / PPL'
                set key outside below
            	plot 'figures/data/bart_sncr.csv' u 8:9 w linespoints title 'F1' axis x1y1, \
                     'figures/data/bart_sncr.csv' u 8:10 w linespoints title 'ROGUE1' axis x1y1, \
                     'figures/data/bart_sncr.csv' u 8:11 w linespoints title 'ROGUE2' axis x1y1, \
                     'figures/data/bart_sncr.csv' u 8:12 w linespoints title 'ROGUEL' axis x1y1, \
                     'figures/data/bart_sncr.csv' u 8:13 w linespoints title 'BLEU' axis x1y2, \
                     'figures/data/bart_sncr.csv' u 8:19 w linespoints title 'PPL' axis x1y2
                
            \end{gnuplot}
            \caption{Generation}
            \label{fig:sncr-generation}
        \end{subfigure}
        \caption{Effectiveness of $\sncr$}
        \label{fig:sncr}
    \end{figure}    


==> sections/discussions.tex <==
\section{Discussion}
\subsection{Base Language Model Choice}
\label{sec:discussion:base-lm}
The \ourmethod method presented in this paper, follows the same framework as the baselines, allowing for the use of any type of language embedding model $(LM)$. Although determining the optimal architecture for a specific problem remains challenging~\cite{fu2023decoder}, numerous studies have shown that decoder-only models ~\cite{radford2019gpt2} are better suited for open-ended generation (such as creative writing), while encoder-only models~\cite{devlin2018bert} are more effective for understanding and summarizing text (such as text classification). Encoder-decoder models~\cite{lewis2019bart} are best for tasks that require the strengths of both (such as question answering). Therefore, the GPT2 (decoder-only) model is not suitable for the problem defined in Section~\ref{sec:method}, which requires both comprehensive summarization of the language in PG/KG networks and open-ended generation tasks. Experimentally, all methods (including ours and baselines) with GPT2 as the base $LM$ produced unsatisfactory results. Therefore, we focused our analysis on methods based on the BART model, which employs an encoder-decoder architecture.
%

\subsection{Computational Efficiency}
\label{sec:discussion:efficiency}
The \ourmethod method employs sparse sampling on tokens for \ssncolbertsim similarity. In theory, it should enhance efficiency by reducing computations for pairwise token similarity. However, we observed that \ourmethod incurs $\sim5\%$ additional time overhead in both training and inference compared to baseline methods. We attribute this efficiency issue to the on-the-fly computation of term frequency, which necessitates constant data transfer between CPU and GPU. Although this performance penalty is relatively small, we aim to improve the efficiency of our approach in future research.

%TODO: Junfeng these kind of promises are not allowed. So, modified the sentance as above.
%At the time of submission, we are actively working on optimizing our implementation for TF-IDF weights to improve computational efficiency. We will share updated results following the anonymous review process.


% \subsection{Low-level Word Interaction}
% \label{sec:discussion:low-level}

% Although Liu~\etal~\cite{liu2023context} demonstrated the value of low-level word similarities in knowledge graph (KG) networks, earlier works (\cite{liu2023context} and \cite{jang2022call})  neglected persona label imbalance. Our work addressed this issue by employing weighting and sampling strategies and confirmed the benefit of word similarities for both KG and persona graph (PG) networks.

%The previous work of Liu~\etal~\cite{liu2023context} has indicated that leveraging low-level word similarities is helpful in the KG network. As mentioned in Section~\ref{sec:method:generation}, both \cite{liu2023context} and \cite{jang2022call} failed to address the persona label imbalance issue and their PG networks were overfitted (\pkfocus$^0$ and \pkncli$^0$). Our experiments on \pkfocus and \pkncli with the persona label weighting and sampling strategies has not only address the issue for both method, but also affirmed the conclusion for both KG and PG networks that leveraging low-level word similarity helps better find the relevant entries and improve the response generation quality.  

% Editing finished by Raju, 7/14/24


